The Convex Geometry of Network Flows

In this paper, we derive a number of interesting properties and extensions of the convex flow problem from the perspective of convex geometry. We show that the sets of allowable flows always can be imbued with a downward closure property, which leads to a useful `calculus' of flows, allowing easy combination and splitting of edges. We then derive a conic form for the convex flow problem, which we show is equivalent to the original problem and almost self-dual. Using this conic form, we consider the nonconvex flow problem with fixed costs on the edges, i.e., where there is some fixed cost to send any nonzero flow over an edge. We show that this problem has almost integral solutions by a Shapley--Folkman argument, and we describe a rounding scheme that works well in practice. Additionally, we provide a heuristic for this nonconvex problem which is a simple modification of our original algorithm. We conclude by discussing a number of interesting avenues for future work.

==> scratch.tex <==
\section{Projected L-BFGS}\label{app:lbfgs}
\TD{NOTE: Not used. Saving to put some of this in the algorithms paper...}
We solve the convex flow problem~\eqref{eq:main-problem} by solving the 
dual problem~\eqref{eq:dual-problem} and then finding a primal feasible solution, 
as outlined in~\S\ref{sec:dual-primal-feas}. To solve the dual problem, we use 
the a projected variant of the L-BFGS algorithm~\cite{} inspired by~\cite{}. 
Beginning from a dual-feasible point, this algorithm constructs a sequence of
dual-feasible iterates such that the objective value of the dual function 
decreases at each iteration. Importantly, the algorithm's performance is 
governed by subroutines that can be efficient implemented and parallelized,
taking advantage of the network structure present in the original problem.
\TD{Add note about L-BFGS on nonsmooth problems? Handle with a bundle method?}

Recall that, when we take into account implicit constraints, the dual problem~\eqref{eq:dual-problem} 
can be written as
\[
\begin{aligned}
    & \text{minimize} && \bar U(\nu) + \sum_{i=1}^m \left(\bar V_i(\eta_i - A_i^T\nu) + f_i(\eta_i)\right) \\
    & \text{subject to} && \eta_i \ge A_i^T\nu, \quad i = 1, \dots, m \\
    &&& \nu \ge 0.
\end{aligned}
\]
For the sake of exposition, we will write this problem as
\[
    \begin{aligned}
        & \text{minimize} && g(\mu) \\
        & \text{subject to} && \mu \in K = \{ \mu \mid F\mu \ge 0\},
    \end{aligned}
\]
where $\mu = (\nu, \eta) \in \reals^n \times \reals^{\sum_{i=1}^m n_i}$ and $B$ 
is matrix that encodes the constraints. Note that a point $\mu^\star$ is optimal
if and only if
\begin{equation}
    \label{eq:lbfgs-opt}
    \nabla g(\mu^\star) \in K^\star = \{ F^T\lambda \mid \lambda \ge 0\},
\end{equation}
where $K^\star$ denotes the dual cone of $K$, defined as 
\[
    K^\star = \{ y \mid y^Tx \ge 0 ~ \text{for all} ~ x \in K\}.
\]
The characterization of the dual cone follows from Farkas' 
Lemma~\cite[\S2.3.1]{}. In terms of variables with the same dimensions
as the original problem, the dual cone can be written as
\[
    K^\star = \left\{
        \left(
            \lambda_1, \dots, \lambda_m,\, 
            \zeta - {\textstyle\sum_{i=1}^m A_i\lambda_i}
        \right)
        \mid
        \zeta \in \reals^n_+,\;
        \lambda_i \in \reals^{n_i}_+,\; i = 1, \dots, m
    \right\}.
\]

To run the projected L-BFGS algorithm, we need three subroutines: a function 
evaluation for $g$, a gradient evaluation for $g$, and a projection onto $K$,
which is easily seen to be a polyhedral cone. The function evaluation for $g$
is simply the evaluation of the dual function~\eqref{eq:dual-function}, which
relies on the subroutines for the subproblems~\eqref{eq:subproblems}. The
gradient can be computed directly from the solutions to these subproblems, as in~\eqref{eq:gradient}.
(Of course, when not at optimality, these gradients will not be zero.)
% We discuss these subroutines after
% outlining the overall algorithm.
% \TD{Can project the gradient, search direction, or final iterate. }
At each iteration $k$, we compute (1) a feasible quasi-Newton search direction 
$p_k$, (2) a step size $\alpha_k$, and (3) the next iterate $\mu_{k+1}$. 
% found by projecting $\mu_k + \alpha_k p_k$ onto the constraint set $K$. 
Thus, each iteration has the form
\[
    \mu_{k+1} = \mu_k + \alpha_k p_k,
\]
Note that, since $p_k$ is feasible ($p_k \in K$) and
the initial iterate is assumed to be feasible, the iterates
$\mu_k$ are always feasible, which follows directly from the definition of $K$.

\paragraph{Termination.}
We terminate the algorithm when the optimality condition~\eqref{eq:lbfgs-opt} is
approximately satisfied. We declare a point $\mu$ optimal and terminate the 
algorithm in two scenarios. First, if the gradient $\nabla g(\mu)$ is sufficiently 
close to zero for $\mu$, which we measure with the $\ell_\infty$ norm. Second, if
$\mu$ is on the boundary of $K$ and the condition~\eqref{eq:lbfgs-opt} approximately
holds. This condition can be checked efficiently if we have access to a projection
onto $-K$ because
\[
    \Pi_{K^\star}(\nabla g(\mu)) = \nabla g(\mu) - \Pi_{-K}(\nabla g(\mu))
\]
by the Moreau decomposition~\cite{}. This subroutine follows almost immediately
from the projection onto $K$, which we discuss shortly. Again, we measure
closeness by the $\ell_\infty$ norm. See the documentation for default tolerances.

\subsection{Algorithm}
We briefly describe the projected L-BFGS algorithm. For more details and additional
implementation considerations, see~\cite[\S7.2]{}. First, the search direction
$p_k$ is computed as
\[
    p_k = \Pi_K\left(-H_k\nabla g(\mu_k)\right),
\]
where $H_k$ is an approximation to the inverse Hessian of $g$ at $\mu_k$.

\paragraph{Hessian approximation.}
Define the vectors
\[
    s_k = \mu_{k+1} - \mu_k = \alpha_kp_k, \quad \text{and} 
    \quad y_k = \nabla g(\mu_{k+1}) - \nabla g(\mu_k).
\]
The BFGS update finds the matrix $B_{k+1}$ the (symmetric) matrix closest to 
$H_k$ that satisfies secant equation, $B_{k+1}s_k = y_k$~\cite{XXX}. This matrix
is given by
\[
    B_{k+1} = \left(I - \rho_k s_ky_k^T\right)H_k\left(I - \rho_k y_ks_k^T\right) + \rho_k s_ks_k^T,
\]
where $\rho_k = 1/(y_k^Ts_k)$. This matrix is usually dense, so L-BFGS stores a
modified version of this matrix implicitly, by taking $B_{k-M} = I$ and storing
only the vectors $s_k$ and $y_k$ for $k = k-M, \dots, k-1$, where positive 
integer $M$ is the \emph{memory} size. (Usually $M$ is taken to be small, for
example $5$ or $10$.) With this implicit representation, the quantity $-H_k\nabla g(\mu_k)$ 
can be computed in $O(M(n + \sum_{i=1}^m n_i))$ time, which is linear in the 
number of variables.
\TD{Add cites (e.g., [HAG17; HHY18]), from Akshay paper}

\paragraph{Seach direction.}
To obtain a search direction $p_k$, we must project negative preconditioned 
gradient $H_k\nabla g(\mu_k)$ onto the constraint set $K = \{ \mu \mid F\mu \ge 0\}$. 
This projection can be computed very efficiently due to the special structure of 
the projector matrices $A_i$. We defer the discussion of this subroutine until~\S\ref{sec:projection}. 
Importantly, after projection, this search direction will be (dual) feasible and, 
therefore, result in a feasible next iterate $\mu_{k+1}$, given that the previous 
iterate $\mu_k$ is feasible. Since we can set the initial iterate $\mu_0$ to be 
feasible (\eg, by choosing $\mu_0 = \ones$), we can guarantee that all iterates 
$\mu_k$ will be feasible.

\paragraph{Step size.}
Finally, to compute the next iterate
\[
    \mu_{k+1} = \mu_k + \alpha_k p_k,  
\]
we choose a step size $\alpha_k$ that 
satisfies the strong Wolfe conditions~\cite[\S]{nocedalNumericalOptimization2006}:
\begin{equation}\label{eq:strong-wolfe}
\begin{aligned}
    g(\mu_k + \alpha_k p_k) &\le g(\mu_k) + c_1\alpha_k \nabla g(\mu_k)^Tp_k, \\
    \abs{\nabla g(\mu_k + \alpha_k p_k)^Tp_k} &\le c_2 \abs{\nabla g(\mu_k)^Tp_k}.
\end{aligned}
\end{equation}
We use the values $c_1 = 10^{-4}$ and $c_2 = 0.9$ from~\cite[\S3]{nocedalNumericalOptimization2006}.
The first condition, sometimes called the Armijo condition, stipulates that the
function value must decrease sufficiently after the step. The second condition
ensures that the step does not take us far from a local minimizer along the 
search direction. We find a step size $\alpha_k$ that satisfies~\eqref{eq:strong-wolfe}
via the Hager-Zhang line search~\cite{XXX} from the \texttt{LineSearches.jl}
package~\cite{XXX}. Importantly, this line search is robust to numerical
precision issues.


\paragraph{Restarts.} 
One potential issue with this method is that our trial direction $-H_k\nabla g(\mu_k)$
may be orthogonal to the constraint set $K$, \ie,  
\[
    -H_k\nabla g(\mu_k) \in K^\star.
\]
(The gradient itself, however, may not necessarily lie in the dual cone).
In this case, the search direction $p_k = 0$, and the algorithm may stop making 
progress. As a result, if we detect that the search direction is approximately
zero, we restart the Hessian approximation, using $H_{k+1} = I$. If, after a 
restart, we find that 
\[
    -H_{k+1}\nabla g(\mu_{k+1}) =  -\nabla g(\mu_{k}
\]
is in the dual cone, we terminate the algorithm and declare the current iterate
$\mu_{k+1}$ optimal. Otherwise, we continue with the algorithm as normal.


\subsection{Projection onto $K$}\label{sec:projection}
In this section, we outline the efficient projection operation onto the cone $K$
used in our software. Recall that the cone $K$ is defined by the following 
inequalities:
\[
    \begin{aligned}
        \eta_i &\ge A_i^T \nu, \quad i = 1, \dots, m, \\
        \nu &\ge 0.
    \end{aligned}
\]
The projection of the point $(\tilde \nu, \tilde \eta_1, \dots, \tilde \eta_m)$ 
onto this set is the minimizer of the optimization problem
\[
\begin{aligned}
& \text{minimize} &&  \sum_{j=1}^n(\nu_j - \tilde \nu_j)^2 + 
\sum_{i=1}^m  \sum_{j=1}^{n_i}(\eta_{ij} - \tilde \eta_{ij})^2 \\
& \text{subject to} && \eta_i \ge A_i^T \nu, \quad i = 1, \dots, m, \\
&&& \nu \ge 0.
\end{aligned}
\]
Our algorithm will use the fact that the matrices $A_i$ are indexers and this
problem is separable. Instead of grouping the objective and constraints by 
edges, we will group them by nodes and split this problem into $n$ smaller problems,
one for each node. Define $N_j$ as the set of edge-local index pairs of edges
adjacent to node $j$:
\[
    N_j = \{(i, k) \mid (A_i)_{kj} = 1 ~ \text{for some} ~ 
i \in \{1, \dots, m\} ~ \text{and} ~ k \in \{1, \dots, n_i\}\}.
\] 
The projection problem can be written as 
\[
\begin{aligned}
& \text{minimize} && \sum_{j=1}^n \left(
    (\nu_j - \tilde \nu_j)^2 + 
    \sum_{(i,k) \in N_j} \left((\eta_i)_k - (\tilde\eta_i)_k\right)^2 
\right) \\
& \text{subject to} && (\eta_i)_k \ge \nu_j, ~ \text{for all} ~ (i,k) \in N_j, \quad j = 1, \dots, n, \\
&&& \nu_j \ge 0, \quad j = 1, \dots, n.
\end{aligned}
\]
Clearly, this problem separates into $n$ independent problems, one for each node,
which can be solved in parallel. These problems have the form
\[
\begin{aligned}
&\text{minimize} && (u - \tilde u)^2 + \sum_{l = 1}^{\abs{N_j}} (w_l - \tilde w_l)^2 \\
&\text{subject to} && w_l \ge u, \quad l = 1, \dots, \abs{N_j}, \\
&&& u \ge 0,
\end{aligned}
\]
where we assume that $w$ is ordered such that $w_1 \le \cdots \le w_{\abs{N_j}}$.
An optimal solution to this problem is given by an average of all the points that
are changed by the projection. In particular, the solution will be of the form
$u^\star = \tau \ge 0$ and
\[
    w^\star_i = \begin{cases}
        \tilde w_i & \text{if} ~ \tilde w_i > \tau \\
        \tau & \text{if} ~ \tilde w_i \le \tau,
    \end{cases}
\]
with corresponding objective value
\[
    (\tau - \tilde u)^2 + \sum_{l = 1}^{\abs{N_j}} (\tau - \tilde w_l)_+^2.
\]
The solution is therefore given by the average of the points that are `included'
in the above sum. Since this is a univariate convex optimization problem with a
closed form solution, and the number of edges incident to any node is usually
small, a simple strategy is to just iterate through the solution until the 
objective value stops decreasing. 

In particular, find the first index $l'$ such that $\max(0, w_{l'}) > 0$. Then
for $l = l', \dots, \abs{N_j}$ compute the average
\[
    \tau = \frac{1}{l + 1}\left(
        \tilde u + \sum_{l'' = 1}^{l} \tilde w_{l''} \right)
\]
If $\tau > w_{l+1}$, we clearly must include this point in the average and we
increase $l$. Otherwise, the optimality conditions of this subproblem are
satisfied and we can stop. The average can be incrementally updated, so the
solution to this problem only requires $O(\abs{N_j})$ additions. Furthermore,
this problem can be parallelized for all of the $n$ nodes.


